Properties of Neutron Star Critical Collapses

Critical phenomena in gravitational collapse opened a new mathematical vista into the theory of general relativity and may ultimately entail fundamental physical implication in observations. However, at present, the dynamics of critical phenomena in gravitational collapse scenarios are still largely unknown. My thesis seeks to understand the properties of the threshold in the solution space of the Einstein field equations between the black hole and neutron star phases, understand the properties of the neutron star critical solution and clarify the implication of these results on realistic astrophysical scenarios. We develop a new set of neutron star-like initial data to establish the universality of the neutron star critical solution and analyze the structure of neutron star and neutron star-like critical collapses via the study of the phase spaces. We also study the different time scales involved in the neutron star critical solution and analyze the properties of the critical index via comparisons between neutron star and neutron star-like initial data. Finally, we explore the boundary of the attraction basin of the neutron star critical solution and its transition to a known set of non-critical fixed points.

==> abbreviations.tex <==
\lhead{}
\rhead{\textit{Abbreviations}}
\begin{abbreviations}
\end{abbreviations}



==> dedication.tex <==
\pagestyle{plain}
{\em to my father and mother for their infinite love and support}


==> introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\chapter{Introduction}
\label{chap:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
Gravitational wave astronomy and high-energy astrophysics are two emerging areas of modern astronomy. Although scientists in these two fields observe our universe by detecting different signals: one gravitational and the other electromagnetic, their theoretical models depend on the general theory of relativity, originated from Albert Einstein. Furthermore, high-energy radiation (X-ray, ${\gamma}$-ray) is often emitted in regions of strong gravitational fields near compact objects, such as neutron stars (NSs) and black holes (BHs), which are usually sources of gravitational radiation as well~\cite{Piran04}. However, due to the complexity of the Einstein field equation (EFE), it is impractical to get exact solutions to the EFE to model the realistic astrophysical problems analytically. Under the circumstances when the gravitational field is weak or not so dynamic, approximation theories, such as the perturbation and post-Newtonian theories, are applied. Nevertheless, when the gravitational field is strong and dynamic, the approximation theories will not work and the Einstein equations can only be solved numerically with the aid of computers. After years of development, the art and science involved in reformulating and numerically solving the EFE has evolved into a new field, numerical relativity.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\section{Brief history of numerical relativity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
As early as the 1920s, not long after Einstein published his paper on the general theory of relativity in 1916, Darmois originated the $3+1$ formalism, which was further developed by Lichnerowicz and Choquet-Bruhat~\cite{Gourgoulhon07}. In the late 1950s, Dirac reformulated the EFE into the Hamiltonian formulations \cite{Dirac58}. Arnowitt, Deser and Misner (ADM) published the ADM $3+1$ formalism \cite{ArnowittDM62} in 1962. The basic idea of the formalism is to split the time coordinate from the spatial coordinates and recast the equations into a set of constraint equations and a set of evolution equations. Since it is physically intuitive and the evolution scheme can be easily implemented numerically, the ADM formalism was widely used in 1960s and 1970s. The first numerical studies of the Einstein field equations with $3+1$ formalism were achieved in the mid 1960s. Hahn and Lindquist simulated the axis symmetric collision of two black holes \cite{HanhL64}. Podurets \cite{Podurets64} in the USSR and May and White \cite{MayW66} in the United States studied the star collapse problem. Early attempts to solve Einstein equations numerically suffered from problems with long-term instability and lack of accuracy. The lack of accuracy is mainly because there were not so many decent numerical schemes and advanced computing technology in those early days, while there are many reasons why the long-term evolution becomes unstable.

One of the reasons lies within the standard ADM formalism, whose direct numerical implementation was proved unstable \cite{Miller00}. There are many variants of the standard ADM formalism aiming to improve the stability. The most successful one to date is the so called {\em Baumgarte-Shapiro-Shibata-Nakamura (BSSN)} scheme \cite{ShibataN95, BaumgarteS99}, which was proposed by Shibata and Nakamura in 1995 \cite{ShibataN95} and slighted modified by Baumgarte and Shapiro in 1999 \cite{BaumgarteS99}. Since the BSSN formalism shows superior stability properties, it has been widely used. The research work done in this dissertation is mainly based on the BSSN formalism, and we will further discuss it in Section~\ref{sec:bssn}. Following Garfinkle's idea of the generalized harmonic gauge \cite{Garfinkle02}, Pretorius proposed and numerically implemented the {\em generalized harmonic decomposition scheme} that is based on the harmonic decomposition of the Ricci tensor and successfully simulated BH binaries, which is the first complete binary BH simulation, from orbit to ringdown together with GW extractions \cite{Pretorius05a,Pretorius05b,Pretorius06}. So far, the generalized harmonic decomposition scheme has mainly been used in BH simulations, and we will not discuss it in this work. Please refer to \cite{Pretorius05a,Pretorius05b,Pretorius06} for details. 

Another reason why the early numerical codes crashed very early during the evolution is due to the formation of the coordinate singularities. To simplify the final formulations, early numerical implementations usually chose very simple gauge conditions. In the case where strong and dynamic gravitational fields are involved, the numerical codes would not be able to handle the strongly stretched hypersurfaces and dragged spatial coordinates. Studies done by Smarr and York in 1970s showed that one can use proper dynamic gauge choices to avoid coordinate singularities \cite{SmarrY78a,York79}. Many slicing conditions and coordinate evolution choices have been proposed and tested so far. We will discuss them in detail in Section~\ref{sec:gauge}.

The initial value problem in GR was studied along with the development of the $3+1$ formalism. Lichnerowicz \cite{Gourgoulhon07} first proposed the conformal decomposition method, which decomposes the spatial metric $\gamma_{ij}$ on the initial hypersurface into a conformal factor and a conformal metric,
\begin{equation}
\gamma_{ij} = \psi^{4} \tilde{\gamma}_{ij},
\end{equation}
where $\psi$ is the conformal factor and $\tilde{\gamma}_{ij}$ is the conformal metric. Choquet-Bruhat and York \cite{York71,York99} extended Lichnerowicz's idea and built the theoretical foundation for most of the numerical implementations to get initial data. The idea of conformal decomposition was also suggested to be helpful in evolution since the true degrees of freedom of the gravitational field are carried by the conformal 3-metric as shown by York \cite{York71,York72a}. As we will see in Section~\ref{sec:bssn}, the success of the BSSN evolution scheme is largely due to the conformal decomposition. There have been several methods developed to provide initial data, such as the conformal transverse-traceless (CTT) method \cite{Gourgoulhon07, York71, York72a, York72b}, the conformal thin sandwich (CTS) method \cite{York99} and the extended conformal thin sandwich (XCTS) method \cite{PfeifferY03}. In order to provide initial data for binary systems, Baumgarte etc. proposed the conformally flat quasiequilibrium (CFQE) approach \cite{BaumgarteCSST97, BaumgarteCSST98b}, which has been widely used to construct compact binary initial data. Detailed reviews on initial value problems in general relativity can be found in \cite{York79,ChoquetY80,Cook00} and the references therein.

Besides the $3+1$ formalism we describe above, the characteristic decomposition method first proposed by Bondi in 1960 \cite{Bondi60}, is also often used to dissemble the EFE. The basic idea of the method is to use characteristic hypersurfaces instead of spatial hypersurfaces in ADM ``3+1'' formalism. The characteristic formalism does not put constraints on the initial data while leaving little room for gauge choices. It is suited to studying radiation problems since the boundary surfaces are null surfaces and there is no extraneous outgoing radiation condition or other artificial boundary conditions necessary. The $2+2$ method proposed by d'Inverno and Smallwood\cite{DinvernoS80} is very close to the characteristic method. The basis of the $2+2$ method is to decompose the spacetime into two families of spacelike 2D surfaces. An initial 2D submanifold is chosen together with two vector fields that translate the submanifold everywhere. Despite the theoretical advantages in many aspects, the characteristic approach suffers from the formation of caustics in the light rays generating the null hypersurfaces. The details of the characteristic type approaches and some of their applications can be found in \cite{Winic05} and the references therein.

For spacetimes with a Killing vector field, namely with an internal symmetry, Geroch proposed to single out the Killing direction and decompose the remaining 3D hypersurfaces in to a 2+1 form with the ADM approach in 1971 \cite{Geroch71}.

Based on the Regge calculus, Regge proposed a lattice formulation of the EFE \cite{Regge61} in 1961 and later developed by many researchers~\cite{WilliamsT92,Gentle02}. Instead of differentiable manifold, Regge calculus reformulates GR with a piecewise flat simplicial complex, which is the four dimensional generalization of triangles and tetrahedra in general. The interior of each three and four dimensional lattice element is intrinsically flat, with curvature concentrated on the two-dimensional faces (triangles). More information about the Regge calculus and its applications can be found in \cite{WilliamsT92, Gentle02} and references therein.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\section{Motivation}
\label{sec:motivation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
Coalescing binary NSs are considered to be strong candidates as sources of GWs detectable by both the existing ground-based detectors such as LIGO, VIRGO, GEO600, and TAMA300 and the proposed space-based detector LISA \cite{CulterT02}. Some studies also propose that coalescing binary NSs are the sources of short ${\gamma}$-ray burst (GRB) detected by advanced ${\gamma}$-ray observatories, CGRO (the Compton Gamma-Ray Observatory), HETE II \cite{Piran04}. Numerical studies of the coalescing binary neutron star system will give us a better understanding of the problem as well the physics underneath.

The acquisition of accurate theoretical waveforms plays an important role in the successful detections of GWs. In order to extract physical information in detected waveforms, template matching techniques are commonly used: detected waveforms are cross-correlated to theoretical ones with known physical properties stored in the GWs bank. Usually, different methods are used to calculate GWs during different phases. When two stars in a binary system have a large separation, or in the inspiral phase, they can be treated as two point masses and their equations of motion, as well as gravitational radiations, can be very accurately calculated with post-Newtonian methods \cite{Blanchet06}. When the orbit shrinks to the so-called innermost stable circular orbit (ISCO) and enters the coalescent phase, two stars begin to plunge and merge. The gravitational fields are so strong and dynamic when two NSs merge that the full EFE is required to model the coalescing binary NSs correctly. Meanwhile, the deformation of two stars in the coalescence stage makes it necessary to utilize the hydrodynamic model of NSs instead of treating them as point masses. Due to the complexity of the fully general relativistic hydrodynamics equations, the waveforms in the coalescence stage can only be calculated numerically with the aid of computers, usually supercomputers. 

Nevertheless, even with today's most powerful supercomputers, it is still impossible to calculate accurate waveforms with uniform grid finite difference methods due to the huge requirement of computational resources \cite{Miller05}. First, realistic astrophysical phenomena usually requires full $3D$ simulations. Second, the coalescence of two neutron stars involves multiple length scales (see Chapter~\ref{chap:amr}). The numerical simulation must resolve the shortest length scale while having a computational domain that covers the longest length scale.

In this thesis, we utilize the state of the art multi-grid techniques to add recursively extra finer grids to provide the high resolution needed to resolve the neutron star dynamics while maintain a large enough computational domain for the determination of gravitational radiation from the binary inspiral and coalescence. We also investigate the premature collapse conjecture of Wilson et al.. In order to study binary NS systems, the author developed: a numerical module to import and verify spectral initial data set to GR-Astro-AMR, an analysis module for GR-Astro-AMR to calculate the invariant quantities and solve the geodesic equations, and a module to analyze GWs.
